Airphant: Cloud-oriented Document Indexing

Modern data warehouses can scale compute nodes independently of storage. These systems persist their data on cloud storage, which is always available and cost-efficient. Ad-hoc compute nodes then fetch necessary data on-demand from cloud storage. This ability to quickly scale or shrink data systems is highly beneficial if query workloads may change over time. We apply this new architecture to search engines with a focus on optimizing their latencies in cloud environments. However, simply placing existing search engines (e.g., Apache Lucene) on top of cloud storage significantly increases their end-to-end query latencies (i.e., more than 6 seconds on average in one of our studies). This is because their indexes can incur multiple network round-trips due to their hierarchical structure (e.g., skip lists, B-trees, learned indexes). To address this issue, we develop a new statistical index (called IoU Sketch). For lookup, IoU Sketch makes multiple asynchronous network requests in parallel. While IoU Sketch may fetch more bytes than existing indexes, it significantly reduces the index lookup time because parallel requests do not block each other. Based on IoU Sketch, we build an end-to-end search engine, called Airphant; we describe how Airphant builds, optimizes, and manages IoU Sketch; and ultimately, supports keyword-based querying. In our experiments with four real datasets, Airphant's average end-to-end latencies are between 13 milliseconds and 300 milliseconds, being up to 8.97x faster than Apache Lucence and 113.39x faster than Elasticsearch.

==> figures/exp_scalability_zipf.tex <==
\begin{figure}[t]
  \centering

\pgfplotsset{latfig/.style={
    width=1.0\linewidth,
    height=30mm,
    xmin=10000,
    xmax=100000000,
    ymin=0,
    ymax=150,
    % xlabel=$n_w$,
    % ylabel=RMS Error,
    xlabel near ticks,
    ylabel near ticks,
    ylabel style={align=center},
    xtick={1000, 10000, 100000, 1000000, 10000000, 100000000},
    % xtick={0, 10, ..., 100},
    % xticklabels={80\%, 85\%, 90\%, 95\%, 99\%, 99.5\%},
    % yticklabels={0\%, 30\%, 60\%, 90\%, 120\%, 150\%},
    % xticklabel style={rotate=30,yshift=-2mm,anchor=east,xshift=1.5mm},
    % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
    % extra y ticks={10, 20, 30, 40},
    % extra y tick style={yticklabels={}},
    ylabel shift=-2pt,
    xlabel shift=-2pt,
    % legend columns=5,
    every axis/.append style={font=\footnotesize},
    % ymajorgrids,
    % yminorgrids,
    minor grid style=lightgray,
    % nodes near coords,
    % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
}}
  
\pgfplotsset{accfig/.style={
    width=1.0\linewidth,
    height=30mm,
    xmin=1000,
    xmax=100000000,
    ymin=0,
    ymax=150,
    % xlabel=$n_w$,
    % ylabel=RMS Error,
    xlabel near ticks,
    ylabel near ticks,
    ylabel style={align=center},
    xtick={1000, 10000, 100000, 1000000, 10000000, 100000000},
    % xtick={0, 10, ..., 100},
    % xticklabels={80\%, 85\%, 90\%, 95\%, 99\%, 99.5\%},
    ytick={102400, 10485760, 1073741824, 107374182400},
    yticklabels={100KB, 10MB, 1GB, 100GB},
    % xticklabel style={rotate=30,yshift=-2mm,anchor=east,xshift=1.5mm},
    % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
    % extra y ticks={10, 20, 30, 40},
    % extra y tick style={yticklabels={}},
    ylabel shift=-2pt,
    xlabel shift=-2pt,
    % legend columns=5,
    every axis/.append style={font=\footnotesize},
    minor grid style=lightgray,
    minor tick num=1,
    ymajorgrids,
    yminorgrids,
    % nodes near coords,
    % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
}}

\begin{minipage}{\linewidth}
\centering
\begin{tikzpicture}
    \begin{customlegend}[
        % legend entries={SQLite,Lucene,\system-1.0,\system-0.01,\system-0.0001},
        legend entries={SQLite,Lucene,\system},
        legend style={
            at={(0.5,1.1)},anchor=south,column sep=2pt,
            draw=black,fill=none,line width=.5pt,
            /tikz/every even column/.append style={column sep=5pt},
            font=\scriptsize,
            align=left,
        },
        legend columns=3,
    ]
    \addlegendimage{vintageblack,fill=vintageblack,mark=square*}
    \addlegendimage{vintageblack!50,fill=vintageblack!50,mark=diamond*}
    \addlegendimage{vintageorange,fill=vintageorange,mark=*}
    % \addlegendimage{vintageorange!75,fill=vintageorange!75,mark=o}
    % \addlegendimage{vintageorange!50,fill=vintageorange!50,mark=x}
    \end{customlegend}
\end{tikzpicture}
\end{minipage}

\hspace*{-5mm}
\begin{subfigure}{0.49\linewidth}
    \begin{tikzpicture}
    \begin{axis}[latfig,
        xmin=1000,
        xmax=100000000,
        % xticklabels={,,},
        xlabel={Corpus Size ($N$)},
        ymin=0,
        ymax=800,
        ymajorgrids,
        xmode=log,
        ylabel=Latency (ms),
        ]
    
    \addplot[mark=square*,mark size=1.5,mark options={fill=vintageblack,draw=vintageblack},
    thick,draw=vintageblack,
    ]
    table[x=x,y=y] {
    d i x y y+
    1 0 1000.0  77.41731738 198.156146
    2 0 10000.0 77.58385079 222.955814
    3 0 100000.0  129.6302303 320.516115
    4 0 1000000.0 251.1510753 640.893597
    5 0 10000000.0  405.0685597 1185.182803
    6 0 100000000.0 608.2446835 1605.451826
    };
    
    \addplot[mark=diamond*,mark size=1.5,mark options={fill=vintageblack!50,draw=vintageblack!50},
    thick,draw=vintageblack!50,
    ]
    table[x=x,y=y] {
    d i x y y+
    1 4 1000.0  105.0240494 1061.365303
    2 4 10000.0 138.0492522 392.500968
    3 4 100000.0  279.9357025 915.891389
    4 4 1000000.0 756.314464  3960.526501
    5 4 10000000.0  1230.006205 4544.676516
    6 4 100000000.0 2455.686716 8514.787842
    };
    
    \addplot[mark=*,mark size=1.5,mark options={fill=vintageorange,draw=vintageorange},
    thick,draw=vintageorange,
    ]
    table[x=x,y=y] {
    d i x y y+
    1 3 1000.0  177.6596509 1829.479016
    2 3 10000.0 125.9759531 220.422271
    3 3 100000.0  151.1214629 297.240302
    4 3 1000000.0 200.5601164 450.504099
    5 3 10000000.0  267.3325568 804.330773
    6 3 100000000.0 331.6545002 874.795758
    };
    
    % \node[anchor=north west,fill=white,draw=black] at (rel axis cs:0.0,1.0) {dataset: \texttt{zipf}};
    \end{axis}
    \end{tikzpicture}
    
    \vspace{-2mm}
    \subcaption{Search Latency}
    \label{fig:scalability:search}
\end{subfigure}%
%
\begin{subfigure}{0.49\linewidth}
    \begin{tikzpicture}
    \begin{axis}[accfig,
        xmin=10000,
        xmax=100000000,
        ymin=100000,
        ymax=107374182400,
        % ytick={1048576, 16777216, 268435456, 4294967296, 68719476736},
        % yticklabels={1, 16, 256, 4096, 65536},
        ymajorgrids,
        xmode=log,
        ymode=log,
        xlabel={Corpus Size ($N$)},
        ylabel=Size (bytes),
        ]
    
    \addplot[mark=square*,mark size=1.5,mark options={fill=vintageblack,draw=vintageblack},
    thick,draw=vintageblack,
    ]
    table[x=x,y=y] {
    d i x y y+
    1 0 1000.0  147568.0  3057.612046
    2 0 10000.0 1331312.0 3131.896759
    3 0 100000.0  13832304.0  4462.802827
    4 0 1000000.0 156369008.0 15422.307603
    5 0 10000000.0  1580847216.0  127391.928623
    6 0 100000000.0 16159735920.0 1430080.25772
    };
    
    \addplot[mark=diamond*,mark size=1.5,mark options={fill=vintageblack!50,draw=vintageblack!50},
    thick,draw=vintageblack!50,
    ]
    table[x=x,y=y] {
    d i x y y+
    1 4 1000.0  54623.0 3574.503421
    2 4 10000.0 585231.0  3863.219679
    3 4 100000.0  6388081.0 5256.904088
    4 4 1000000.0 75423424.0  19213.155614
    5 4 10000000.0  794340401.0 133086.828953
    6 4 100000000.0 8365417390.0  1167300.754987
    };
    
    \addplot[mark=*,mark size=1.5,mark options={fill=vintageorange,draw=vintageorange},
    thick,draw=vintageorange,
    ]
    table[x=x,y=y] {
    d i x y y+
    1 3 1000.0  108951.0  4668.123582
    2 3 10000.0 1138002.0 4501.601345
    3 3 100000.0  15067711.0  6101.835884
    4 3 1000000.0 162234035.0 16500.001546
    5 3 10000000.0  1694988780.0  133144.170339
    6 3 100000000.0 23842342365.0 2071345.524677
    };
    
    % \node[anchor=north west,fill=white,draw=black] at (rel axis cs:0.0,1.0) {dataset: \texttt{zipf}};
    \end{axis}
    \end{tikzpicture}
    \label{fig:scalability:zipf-storage}
    
    \vspace{-6mm}
    \subcaption{Index Storage Usage}
    \label{fig:scalability:storage}
\end{subfigure}

% \vspace{-2mm}
% \caption{\fixed{Effects of corpus size on avg search latency (top) and index size (bottom). Given a corpus size $X$, synthetic datasets are generated with the numbers of documents and words $n_d = n_w = N = 10^x$: \texttt{diag($x$,$x$,0)}, \texttt{unif($x$,$x$,1)}, and \texttt{zipf($x$,$x$,1)} \tofix{use zipf only}}}
\caption{\fixed{Effects of corpus size on avg search latency (left) and index size (right). Given a corpus size $x$, synthetic datasets are generated with the numbers of documents and words $n_d = n_w = N = 10^x$. Here we show results in the \texttt{zipf($x$,$x$,1)} dataset.}}
\label{fig:scalability}

\vspace{-2mm}
\end{figure}


==> sections/4_1_inverted.tex <==
\section{Inverted Index}
\label{sec:inverted}

\yongjoo{Describe our merged(?) inverted index.}


==> sections/6_discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Discussions}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% example cost calculations on some IaaS/PaaS providers
\subsection{Cost Comparison}
\label{sec:discuss:cost-compare}

\supawit{TODO}

In corpus: \tofix{HDFS}

\system answers a query in $225$ ms, using \tofix{small VM}, a cloud storage bucket storing \tofix{S} bytes of index data, reading $1$ per initialization, reading $r_i = L^{*}$ term lookup for postings lists per query, reading $r_d < ~3k$ for doc retrieval per query.

\tofix{other} answers in $t$ ms, from in-memory index structure containing $S_2$ bytes (or disk?), using \tofix{large enough VM}, 

So then we need $225 / t$ \system Seachers to match the throughput in the worst case where concurrent execution is not allowed (try to match cores between the two?).




Index lots of doc (10TB), relatively small vms,

Latency 300 ms, cheapest config to achieve this.
 - Memory, disk (ssd/hard drive), \#VMs (ElasticSearch)
 - Memory holds $C$ bytes
 - Disk: store $S$ bytes of index, read speed x MB/s, need to read $O(\log S) - C$ per query --> latency




\url{https://cloud.google.com/compute/vm-instance-pricing#n2_predefined}

e2-micro	2	1GB	6.11	1.83	3.85	2.75
e2-small	2	2GB	12.23	3.67	7.7	5.5
e2-medium	2	4GB	24.46   7.34	15.41	11.01
e2-standard-2	2	8GB	48.91	14.67
e2-highcpu-8	8	8GB	144.45	43.33

\url{https://cloud.google.com/storage/pricing}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% multiple ways to query iou sketch
\subsection{Query Variants}
\label{sec:discuss:query-variant}

Apart from full and top-$K$ document retrievals, \system opens up many other manners of retrieval. We list some of them here as potential improvements and as a guide for \system's applications.

% overfetch according to FP bounds
\paragraph{Streaming and Prefetching} Instead of fetching each entire IoU Sketch's postings lists, it is possible to consume them and compute the intersection in a stream fashion. To enable such feature, \system Builder would then need to sort the postings within each list before persisting on cloud storage. Stream has many advantages such as reducing initial latency and peak memory usage. In top-$K$ query, it would also reduce the amount of data to be downloaded. Prefetching for next postings can cut down stream's response time as well.

% fetch subset of layers (accuracy on demand)
\paragraph{Partial Fetching for Variable Accuracy} Given a constructed IoU Sketch, \system Searcher is free to fetch any number of layers to intersect. If it chose to read any a subset of the layer, it could decrease memory usage and improve term index lookup latency at a cost of accuracy and, if demanded, overall search latency.

% fetch subset of layers (straggler)
\paragraph{Partial Fetching for Straggler Mitigation} In a different light, IoU Sketch's layered structure provides a natural way to mitigate stragglers---when a few delayed servers delays the operations as a whole. Specifically, stragglers manifesting in postings list retrieval from cloud storage can significantly delay \system Searcher's term index lookup. Partially fetching some layers can mitigate such problem similarly to \cite{Ananthanarayanan2013} by aborting postings list retrievals that are slower than expected.

% bloom filter + exact membership
\paragraph{Filtering with Bloom Filter} Currently \system Searcher filters out irrelevant documents by directly checking with the query words. To do so, it has to retrieve and parse raw documents which can be costly when each document is very large. A workaround is to build a small Bloom filter for each document that answers whether the document contains a given keyword. Although a Bloom filter is not perfect, it can improve the accuracy, and thus, avoid downloading large irrelevant documents.

% % approximated tag + continuous filtering
% \paragraph{Approximated List Visualization}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% alternatives that were considered
\subsection{Considered Data Structures}
\label{sec:discuss:considered-structure}

Our initial attempts try to modify B-tree into an approximated index structure to reduce cloud fetching at a cost of accuracy. Unfortunately, our two directions fail to do so. They include truncating subtrees and fitting decision tree on embedded keys. Subtree truncation aims to reduce B-tree height by combining document lists under truncated subtree into one. On the hand, we try to embed keys into vectors to learn a sparse dictionary of document lists encoded in a form of decision tree. A query would include fetching embedding function and decision boundaries to reconstruct decision tree nodes. Both approaches fail to accurately approximate the document lists, let alone provide a guarantee on trade-off between cost and error.
